A Consistently Oriented Basis for Eigenanalysis: Improved Directional Statistics

The algorithm derived in this article, which builds upon the original paper, takes a holistic view of the handedness of an orthonormal eigenvector matrix so as to transfer what would have been labeled as a reflection in the original algorithm into a rotation through a major arc in the new algorithm. In so doing, the angular wrap-around on the interval {\pi} that exists in the original is extended to a 2{\pi} interval for primary rotations, which in turn provides clean directional statistics. The modified algorithm is detailed in this article and an empirical example is shown. The empirical example is analyzed in the context of random matrix theory, after which two methods are discussed to stabilize eigenvector pointing directions as they evolve in time. The thucyd Python package and source code, reported in the original paper, has been updated to include the new algorithm and is freely available.

==> arxiv_eigen_shared.tex <==
% ------------------------------------------------------------------------------------------------------
% Imported by the author

\RequirePackage[OT2,T1]{fontenc}

\usepackage{algorithm2e}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsopn}
\usepackage{amssymb}
\usepackage{blkarray}
\usepackage[shortcuts]{extdash}
\usepackage{graphicx}
\usepackage{lipsum}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage[customcolors]{hf-tikz}
\usepackage{xspace}

\usepackage[final]{listings}

% correction for multirow format
\renewcommand{\multirowsetup}{\centering}

\usepackage{epstopdf}

\usepackage[colorlinks]{hyperref}
\hypersetup{
  linkcolor = blue,
  citecolor = blue,
  urlcolor  = blue
}

% hf-tikz
\hfsetfillcolor{blue!10}
\hfsetbordercolor{blue}
\usetikzlibrary{matrix,decorations.pathreplacing,calc,positioning,fit}

% tikz colors -- follows the Brewer `Set2' color theme
\definecolor{C1}{HTML}{66c2a5}
\definecolor{C2}{HTML}{fc8d62}
\definecolor{C3}{HTML}{8da0cb}
\definecolor{C4}{HTML}{e78ac3}
\definecolor{C5}{HTML}{a6d854}
\definecolor{C6}{HTML}{ffd92f}


% code listings setup
%   from https://en.wikibooks.org/wiki/LaTeX/Source_Code_Listings
\lstset{
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\sffamily\small,
                                   % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{gray},% comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  firstnumber=1,                   % start line enumeration with line 1000
  frame=none,                      % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Python,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=none,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{Gray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=5,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{Thistle},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}
%

% hyphenation
\hyphenation{eigen-vector}
\hyphenation{eigen-value}
\hyphenation{eigen-analysis}
\hyphenation{eigen-de-com-po-si-tion}
\hyphenation{de-com-po-si-tion}

\hyphenation{ma-chine}
\hyphenation{learn-ing}
\hyphenation{sin-gu-lar}
\hyphenation{hyper-sphere}
\hyphenation{con-stituent}

